When NAS Meets Trees: An Efficient Algorithm for Neural Architecture Search

The key challenge in neural architecture search (NAS) is designing how to explore wisely in the huge search space. We propose a new NAS method called TNAS (NAS with trees), which improves search efficiency by exploring only a small number of architectures while also achieving a higher search accuracy. TNAS introduces an architecture tree and a binary operation tree, to factorize the search space and substantially reduce the exploration size. TNAS performs a modified bi-level Breadth-First Search in the proposed trees to discover a high-performance architecture. Impressively, TNAS finds the global optimal architecture on CIFAR-10 with test accuracy of 94.37\% in four GPU hours in NAS-Bench-201. The average test accuracy is 94.35\%, which outperforms the state-of-the-art. Code is available at: \url{https://github.com/guochengqian/TNAS}.

==> workshop_sections/ablation.tex <==
\section{Ablation Study}
% We conduct ablation study to show the effectiveness of the architecture tree and the binary operation tree on NAS-Bench-201 benchmark. We also show that any exploitation-reducing methods can be applied with TNAS to further improve the efficiency. 


\subsection{Ablation on Architecture Tree $\mathcal{T}_A$}
$\mathcal{T}_A$ is proposed to reduce the exploration size from $M^L$ to $\lceil\frac{L}{d_a}\rceil \times M^{d_a}$. Here, we experiment with the expansion depth $d_a$ and the construction of the architecture tree (the branching order of the architecture layers). 

\mysection{Expansion depth $d_a$.} 
In Table \ref{table:expand_depth}, we compare TNAS using different expansion depths of the BFS in $\mathcal{T}_A$, ranging from $d_a=0$ to $d_a=L=6$. A larger expansion depth generally leads to a higher search accuracy, but at the cost of search efficiency. It is worthwhile noting that TNAS with $d_a=2$ outperforms GDAS~\cite{dong2019searching}, while using $6\times$ less GPU hours. 

\begin{table}[!htb]
    \centering
    \caption{\textbf{Ablate expansion depths} ($d_a, d_o$) of $\mathcal{T}_A, \mathcal{T}_O$}
    \label{table:expand_depth}
    \vspace{-1em}
    \resizebox{1.\columnwidth}{!}{
    \begin{tabular}{lcccccc}
    \toprule
    \textbf{expansion depth} & \textbf{CIFAR-10} & \textbf{CIFAR-100} & \textbf{ImageNet-16-120} & \textbf{cost (hours)}\\ \midrule
	$d_a=1, d_o=1$ & 93.65$\pm$0.14 & 70.63$\pm$0.37 & 44.57$\pm$0.45 & 1.5\\
	$d_a=1, d_o=3$ & $93.58\pm0.32$ &	$70.96\pm1.23$ & $44.61\pm1.60$  & 1.4\\
	\midrule
	$d_a=2, d_o=1$ & 93.66$\pm$0.20 & 70.93$\pm$0.92 & 44.38$\pm$0.99 & 1.2\\	
	$d_a=2, d_o=3$ &	93.53$\pm$0.43 & 70.94$\pm$1.32	& 44.31$\pm$1.23 & 2.3 \\ 
	\midrule 
	$d_a=3, d_o=1$ & 93.80$\pm$0.09  & 71.64$\pm$0.05 & 45.25$\pm$0.84 & 1.8\\	
	$d_a=3, d_o=3$ & 93.83$\pm$0.17&	70.85$\pm$0.07 & 	44.92$\pm$1.27 &5.3\\
    \midrule
	$d_a=4, d_o=1$ & 94.15$\pm$0.24 & 72.61$\pm$0.94 & 45.97$\pm$0.75 & 2.3\\\midrule
	$d_a=5, d_o=1$ & 94.12$\pm$0.14 & 72.63$\pm$0.50 & 46.02$\pm$0.57	 & 3.1\\\midrule
	\textbf{$d_a=6, d_o=1$} & \textbf{94.35}$\pm$0.03 & \textbf{73.02}$\pm$0.34 & \textbf{46.31}$\pm$0.24& 3.6 \\
    \bottomrule
    \end{tabular}
    }
%    \vspace{-2mm}
\end{table}


\mysection{Branching order of architecture layers.}
We construct  $\mathcal{T}_A$ by branching the one-shot architecture layer by layer. The branching order will change the structure of $\mathcal{T}_A$.
By default, we branch the architecture layer breadth-wise, namely branch all incoming layers of a node at first, then move to the successor of the node in the topological ordering. Here, we experiment with depth-wise order and random order in Table \ref{table:order} with $d_a=1, d_o=1$. The depth-wise order is to branch one layer of the node at first, move to its successor until the last node, then backtrack to the root node and branch its second layer, and so on. Results show that the branching order does not influence the search accuracy much. 

\begin{table}[!htb]
    \centering
    \caption{\textbf{Ablate branching order of the architecture layers}}
    \vspace{-1em}
    \label{table:order}
    \resizebox{1.\columnwidth}{!}{
    \begin{tabular}{lcccc}
    \toprule
    \textbf{Search Order} & \textbf{CIFAR-10} & \textbf{CIFAR-100} & \textbf{ImageNet-16-120}\\ \midrule
	breadth-wise (default) & 93.65$\pm$0.14 &70.63$\pm$0.37 &  44.57$\pm$0.45 \\	
	depth-wise & 93.74$\pm$0.10 &71.52$\pm$0.57& 45.31$\pm$0.86 \\	
	random & 93.70$\pm$0.22 & 70.78$\pm$1.09 & 44.80$\pm$1.20\\	
    \bottomrule
    \end{tabular}
    }
\end{table}



\subsection{Ablation on Binary Operation Tree $\mathcal{T}_O$}\label{sec:ablate_op}
As mentioned earlier, $\mathcal{T}_O$ is proposed to reduce the exploration size from $M^L$ to $\left\lceil\frac{\log_2(M-1) + 1}{d_o} \right \rceil\times 2^{d_oL}$. Here, we experiment with the expansion depth $d_o$ and the construction of $\mathcal{T}_O$ (the grouping strategy of operations). 

\mysection{Expansion depth $d_o$.}
Table \ref{table:expand_depth} shows the influence of the expansion depth $d_o$ of BFS in the binary operation tree $\mathcal{T}_O$. When $d_a$ is small, TNAS tends to be more greedy and favors a smaller $d_o$. When $d_a$ is large, TNAS tends to be more like a global optimizer and favors a larger $d_o$. Overall, the influence of $d_o$ is not as profound as that of $d_a$. 


\mysection{Grouping strategy of operations.}
How operations are branched in $\mathcal{T}_O$ will change the tree's structure. For simplicity, we number the operations in NAS-Bench-201 as (0) $none$, (1) $skip~connection$, (2) $1\times1~conv$, (3) $3\times3~conv$, and (4) $3\times3 ~avgpool$. Our $\mathcal{T}_O$ has a straightforward structure,  $[0, [[2, 3], [1,4]]]$, as shown in Figure \ref{fig:operation_tree}. Here, we ablate different structures, and show their results in Table \ref{table:grouping}. Results demonstrate that the structure of $\mathcal{T}_O$ significantly influences the search accuracy. Our default structure tends to have more distinguishable exclusive operation groups, and is the most accurate among the variants. 

\begin{table}[!htb]
    \centering
    \caption{\textbf{Ablate the grouping strategy of operations} }
    \label{table:grouping}
    \vspace{-1em}
    \resizebox{1.\columnwidth}{!}{
    \begin{tabular}{lccccc}
    \toprule
    \textbf{Grouping} & \textbf{CIFAR-10} & \textbf{CIFAR-100} & \textbf{ImageNet-16-120}\\ \midrule
    \textbf{$[[2, 3], [1, 4]]$(default)}& \textbf{94.35} $\pm$ 0.03 & \textbf{73.02} $\pm$ 0.34 & \textbf{46.31} $\pm$ 0.24  \\
	$[[2, 1], [3, 4]]$ & 93.63$\pm$0.15 &	70.72$\pm$0.35 & 44.57$\pm$0.31  \\	
	$[2,4], [1,3]$ & 93.11$\pm$0.35 &	69.89$\pm$0.12&	43.40$\pm$0.34 \\
    \bottomrule
    \end{tabular}
    }
%    \vspace{-2mm}
\end{table}

% \subsection{Ablation on Exploitation}
% training less epochs.
% weight-sharing. 
% without training.
% \todo{add angle-based; imagenet.}. 

